Optical properties of MoSe$_2$ monolayer implanted with ultra-low energy Cr ions

The paper explores the optical properties of an exfoliated MoSe$_2$ monolayer implanted with Cr$^+$ ions, accelerated to 25 eV. Photoluminescence of the implanted MoSe$_2$ reveals an emission line from Cr-related defects that is present only under weak electron doping. Unlike band-to-band transition, the Cr-introduced emission is characterised by non-zero activation energy, long lifetimes, and weak response to the magnetic field. To rationalise the experimental results and get insights into the atomic structure of the defects, we modelled the Cr-ion irradiation process using ab-initio molecular dynamics simulations followed by the electronic structure calculations of the system with defects. The experimental and theoretical results suggest that the recombination of electrons on the acceptors, which could be introduced by the Cr implantation-induced defects, with the valence band holes is the most likely origin of the low energy emission. Our results demonstrate the potential of low-energy ion implantation as a tool to tailor the properties of 2D materials by doping.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
